STYLER: Style Factor Modeling with Rapidity and Robustness via Speech Decomposition for Expressive and Controllable Neural Text to Speech

Previous works on neural text-to-speech (TTS) have been addressed on limited speed in training and inference time, robustness for difficult synthesis conditions, expressiveness, and controllability. Although several approaches resolve some limitations, there has been no attempt to solve all weaknesses at once. In this paper, we propose STYLER, an expressive and controllable TTS framework with high-speed and robust synthesis. Our novel audio-text aligning method called Mel Calibrator and excluding autoregressive decoding enable rapid training and inference and robust synthesis on unseen data. Also, disentangled style factor modeling under supervision enlarges the controllability in synthesizing process leading to expressive TTS. On top of it, a novel noise modeling pipeline using domain adversarial training and Residual Decoding empowers noise-robust style transfer, decomposing the noise without any additional label. Various experiments demonstrate that STYLER is more effective in speed and robustness than expressive TTS with autoregressive decoding and more expressive and controllable than reading style non-autoregressive TTS. Synthesis samples and experiment results are provided via our demo page, and code is available publicly.

==> 02_method.tex <==
\section{Method}

There are two primary considerations to achieve our goal, non-autoregressive TTS with style factor modeling. First, some non-autoregressive TTS frameworks benefit from supervision, while speech decomposition using bottleneck was studied in an unsupervised condition. Second, as the voice conversion task, the content of audio may not be matched to the text. Prior works \cite{lee2019robust, sun2020fully} hired an attention mechanism, which claimed to be unstable. In this section, we describe the proposed model in detail along with our solution to the aforementioned problems.

\subsection{Model Architecture}

\input{supplementary/model_architecture}

An overview of the proposed architecture is shown in Figure~\ref{fig:figure1}. {\ours} extends FastSpeech2\footnote{https://github.com/ming024/FastSpeech2} \cite{ren2020fastspeech2} and encoders of SpeechSplit\footnote{https://github.com/auspicious3000/SpeechSplit} \cite{qian2020speechsplit} are adapted to take a reference audio as a model input. {\ours} models total six style factors: text, duration, pitch, speaker, energy, and noise. Note that the text is regarded as a style factor equal to audio related ones.

\subsubsection{FastSpeech2 Extension}
For architecture for text encoder and mel-spectrogram decoder, we modified FastSpeech2 \cite{ren2020fastspeech2} to achieve our intent. 
The text encoder has two 256 dimensional Feed-Forward Transformer (FFT) blocks \cite{ren2019fastspeech} with four heads and takes phoneme sequence as input text. We adjust model specifications in order to align the number of parameters with audio encoders. Variance adaptor, including duration predictor, pitch predictor, and energy predictor, is placed on top of the encoders. To become a multispeaker system, speaker encoding is transferred from pre-trained speaker embedding as presented in \cite{jia2018transfer}. In this work, Deep Speaker \cite{li2017deepspeaker} is employed since it is faithful to embed speaker identities without extra features such as noise robustness. 

The decoder has four 256 dimensional FFT blocks with four multi heads. We increase the number of heads since the complexity of decoding would increase to represent variants of style factor combination. The decoder's input is a combination of text encoding, pitch embedding (embedding of pitch predictor output), energy embedding (embedding of energy predictor output), and speaker encoding. Speaker encoding is included because information between input and target should be matched for the desired mapping.

\subsubsection{Speech Decomposition}
We utilize the encoder of SpeechSplit \cite{qian2020speechsplit} to decompose the style factor from source audio. Applying bottleneck onto input, we constrain information fit to target: duration, pitch, or energy.
Each predictor of style factor predicts real value rather than latent code, however, input to each predictor needs to contain all necessary information. Unlike the unsupervised condition, forced feature selection is not needed by virtue of pre-obtained features from incoming audio, and any excessive bottleneck will lead to performance degradation \cite{qian2019autovc}. Therefore, we mitigate the bottleneck to avoid scarcity of information for predictors and relish the supervision.

Basically, we have raw audio as input and extract mel-spectrogram in 80 channels, pitch contour, and energy from it for style factor decomposition. Duration and noise encoder takes mel-spectrogram. Pitch encoder takes a speaker normalized pitch contour (\(mean=0.5\), \(standard~deviation=0.25\)) so that speaker-independent pitch contour is modeled. The energy encoder takes scaled energy from 0 to 1 to ease the model training. After extracted from audio, both pitch, and energy input are quantized in 256 bins one-hot vector, and then processed by encoders.

Each encoder has three 5x1 convolution layers followed by a group normalization \cite{wu2018groupnorm} of size 16 and channel-wise bottleneck by two layers bidirectional-LSTM size 64 except the duration encoder where the size is 80. The dimension of the convolution layer is 256 for duration and noise, 320 for pitch and energy. By linear layer with ReLU activation, encoder outputs are upsampled channel-wise before being sent to each predictor. The content of the audio is removed through the bottleneck in audio-related encoders since the content of the final output of our model should be encoded solely by the text encoder.

The structure of predictors is the same as FastSpeech2. Each predictor takes the sum of the corresponding encoding with text encoding. To balance the dependency, however, the text encoding is projected to four-dimensional space as a channel-wise bottleneck. The pitch predictor receives speaker encoding as an additional input to predict the target speaker's voice with disentangled pitch contour. We project and add speaker encoding to both downsampled and upsampled pitch encoding, finding out empirically that this improves the decomposition of speaker identity.

\subsubsection{\linearmelscaling}
Not using attention alignment, we need to resolve length incompatibility between the content of source audio and input text. Therefore, we apply {\linearmelscaling} between convolution stack and downsampling layer in each style factor encoder.
Asserting length aligning as a frame-wise bottleneck, we design {\linearmelscaling} as a linear compression or expansion of audio to the length of the input text. It simply averages frames or repeats a frame of audio to assign them to a single phone. There are two advantages over the attention mechanism in terms of our objective: it does not bring any robustness issue against the non-autoregressive framework, and it does not being exposed to the text so that audio-related style factors only come from the audio.


\subsection{Noise modeling}

Noise is one of the remaining factors that have been explicitly encoded in model encoders. Therefore, it can be defined based on its residual property, excluding other style factors. In order to model noise by the definition, however, other encoders must be constrained to not include noise information even from noisy input.


\subsubsection{Domain Adversarial Training}
\label{section:dat}

Not including noise information means extracting noise-independent features. In the TTS domain, this has been tackled by applying Domain Adversarial Training (DAT) \cite{ganin2016domain, hsu2019speakercorrelated}. Similarly, in our model, the augmentation label is used to replace the unavailable acoustic condition label (e.g., noise label), and a gradient reversal layer (GRL) is injected to be jointly trainable. The label of each predictor acts as a class label. As shown in Figure~\ref{fig:figure1}, DAT is applied to every audio-related encoding except noise encoder. After passing through GRL, each encoding is consumed by the augmentation classifier to predict the augmentation posterior (original/augmented). The augmentation classifier consists of two fully connected layers of 256 hidden size, followed by layer normalization \cite{ba2016layernorm} and ReLU activation. Note that each encoder except the noise encoder is now noise-independent, so each predictor's output is compared to clean labels rather than noisy ones.


\subsubsection{\doubledecoding}
\label{section:doubledecoding}

According to the definition of noise and the fact that explicit label is not given, the decoder needs to perform {\doubledecoding}: clean decoding and noisy decoding. In clean decoding, all noise-independent encodings are taken to synthesize a clean output, and in noisy decoding, noise encoder output is added to noise-independent encodings to synthesize a noisy output. Since only the noise encoder has to be updated at noisy decoding, the gradient does not flow through the other encoders. It can be seen as implicit supervision where the noise is directly compelled to focus on the audio's leftover part without any explicit label.

\subsection{Loss Calculation}

The total loss of the model without noise modeling is: 
\begin{equation}
    Loss_{clean} = l_{mel}~+~l_{duration}~+~l_{pitch}~+~l_{energy}
    \label{eq:cleanloss}
\end{equation}
where \(l_{mel}\) is mean square error between predicted mel-spectrogram and target, and predictor losses (\(l_{duration}\), \(l_{pitch}\), and \(l_{energy}\)) are calculated by mean absolute error. Note that it is the same as FastSpeech2 which means that the proposed model can disentangle style factors with no additional label.

The loss, including noise modeling, then becomes as follows: 
\begin{equation}
    Loss_{total} = Loss_{clean} ~+~ l_{noisy} ~+~ l_{aug}
    \label{eq:noiseloss}
\end{equation}
where \(Loss_{clean}\) refers to Equation~\ref{eq:cleanloss}, \(l_{noisy}\) is from noisy decoding calculated by the same way of \(l_{mel}\) in Equation~\ref{eq:cleanloss}, and \(l_{aug}\) is the sum of each augmentation classifier loss in Section~\ref{section:dat}.

==> 04_discussion.tex <==
\section{Discussion}

% - 우리는 heuristic하게 noise에 대한 dependency를 고려하지 않은 모델의 style transfer 성능이 더 우수한 것을 확인했음. 즉, DAT와 {\doubledecoding}을 통한 noise 모델링 부분을 제거하고 clean input에서 clean output을 predict하도록 합성하였을 때 성능이 훨씬 잘 나왔음. 이는  noise independent한 특징 추출에 대한 부담이 사라지고, 모델링 하는 요소가 줄어 모든 요소를 동시에 모델링 할 때 훨씬 쉽기 때문임 \cite{qian2020speechsplit}. note that 우리는 모든 style factor modeling을 하면서도 style transfer가 가능했음을 보여주었다는 것이 contribution이었음.
% We heuristically confirmed that the style transfer performance of the model that does not consider the dependency on noise is better. In other words, when the noise modeling part through DAT and {\doubledecoding} was removed and trained to predict clean output from clean input, the performance of style transfer was increased. This is because the burden of noise independent feature extraction disappears and the number of elements to be modeled is reduced, making it much easier to transfer all elements at the same time \cite{qian2020speechsplit}. Note the reason why we were not dealing it is that the objective of our work is not only on style transfer, but also to show the possibility of style factor modeling even with the noise.

% - 기존 FastSpeech2에서도 이미 duration, pitch, energy는 control이 가능했다. 하지만 이들은 text에서만 추측되는 값이었고, 우리 모델의 encoder들은 이를 text와 refernce audio의 필요 요소들에게 의존도를 동등히 분배하는 것이라고 볼 수 있다. 따라서 predictor의 값 (decoder의 input)을 control하는 것과 encoding의 값 (predictor의 input)을 조절하는 것은 약간의 차이가 있다. 예를들어,  duration predictor의 값을 0으로 하면 최종 mel의 frame 길이가 0이 되어 아무것도 합성되지 않지만, duration predictor에 text encoding만 넣으면, audio의 dependency가 제거되어 text가 가지고 있는 기본적인 duration에 기반해 phoneme마다 차이가 거의 없는 일정한 길이의 음성이 합성되게 된다. 여기에 duration encoding까지 넣으면 비로소 text와 audio의 style 모두에 기반한 합성이 이루어 지는 것이다.
We argue that our model's strength over FastSpeech2 is the explicit decomposition of style factor and balanced contribution of style factors, including text content toward synthesized speech. 
In FastSpeech2, the duration, pitch, and energy were already controllable. However, values were only predicted from the text, and the encoders of our model can be seen as distributing the dependence equally among the necessary elements of speech. Therefore, there is a difference between controlling the value of predictors (decoder input) and the encoding (predictor input). For example, if the pitch predictor's value is set to 0, the pitch value of the final mel-spectrogram becomes 0 for each frame. However, if only text encoding is passed to the pitch predictor, the dependency of audio is removed, and the output speech contains almost the same pitch for each phoneme which is not 0. This constant value is the averaged pitch of the training dataset.

% - DAT에서 우리는 DANN \cite{ganin2016domain} 을 사용함. 하지만 최근 Domain Adaptation 기법 \cite{jin2020heuristic}을 적용하면 성능 향상이 가능하고, 이는 우리 모델 novelty와 별개의 문제임.
% On the other hand, we used domain adversarial neural network (DANN) \cite{ganin2016domain} to extract noise-independent features. However, applying the recent Domain Adaptation technique such as \cite{jin2020heuristic} can improve overall performance, which is yet a separate issue from our novelty.

% Noise modeling의 의미
% AS described in Section~\ref{section:dat}, we proved that the noise also can be modeled. It means that we can control noisiness as the same way of others. In other words, noise model predicts different level of the noise depending on the noisiness of input audio. The main contribution of it is that we can explicitly add or remove the noise in the final speech with full control just like the other factors.

% - 우리는 모델의 의존도에 따라 naturalness와 style transfer의 성능에 trade-off가 존재함을 확인하였다. 예를들어, text 의존도를 높이면 naturalness는 올라가지만 reference의 style을 덜 반영하게 되고, 반대로 audio의 의존도를 높이면 reference의 style을 잘 가져오지만 합성된 음성의 naturalness가 떨어졌다. 특히, 이 현상은 duration에서 심하게 나타나서 duration modeling is less clearer than other style factors. 
% On the other hand,  there was a trade-off between the naturalness and style transfer performance according to the model input's dependence. For example, if the text dependency is increased, the naturalness increases too, but the reference style is less reflected. On the contrary, if the audio dependency is increased, the reference style is well transferred, but the naturalness of the synthesized voice decreases. In particular, this phenomenon is severe in duration, so that the duration modeling could be less precise than other style factors.
